Bit Error Robustness for Energy-Efficient DNN Accelerators

Deep neural network (DNN) accelerators received considerable attention in past years due to saved energy compared to mainstream hardware. Low-voltage operation of DNN accelerators allows to further reduce energy consumption significantly, however, causes bit-level failures in the memory storing the quantized DNN weights. In this paper, we show that a combination of robust fixed-point quantization, weight clipping, and random bit error training (RandBET) improves robustness against random bit errors in (quantized) DNN weights significantly. This leads to high energy savings from both low-voltage operation as well as low-precision quantization. Our approach generalizes across operating voltages and accelerators, as demonstrated on bit errors from profiled SRAM arrays. We also discuss why weight clipping alone is already a quite effective way to achieve robustness against bit errors. Moreover, we specifically discuss the involved trade-offs regarding accuracy, robustness and precision: Without losing more than 1% in accuracy compared to a normally trained 8-bit DNN, we can reduce energy consumption on CIFAR-10 by 20%. Higher energy savings of, e.g., 30%, are possible at the cost of 2.5% accuracy, even for 4-bit DNNs.

==> sec_impact.tex <==
\section*{Broader Impact}
On the positive side, this paper aims at increasing robustness of deep neural networks (DNNs) which we consider as an important goal to ensure positive impact of machine learning on our society. In particular, robustness against bit errors, as discussed in this paper, has the potential to lead to improved energy-efficiency of DNN accelerators due to low-voltage operation. Obviously, improved energy-efficiency while maintaining the same prediction performance is a desirable goal.

On the negative side as we are discussing defenses against adversarial manipulation of the DNN weights on a bit-level we also have to discuss attacks to challenge the defense. Thus, we introduce and discuss bit-level adversarial attacks on the weights which, in principle, could be abused to attack an ``undefended'' model. However, this kind of conflict is unavoidable when discussing security relevant issues of machine learning systems.

